Decouple-Then-Merge: Finetune Diffusion Models as Multi-Task Learning

Diffusion models are trained by learning a sequence of models that reverse each step of noise corruption. Typically, the model parameters are fully shared across multiple timesteps to enhance training efficiency. However, since the denoising tasks differ at each timestep, the gradients computed at different timesteps may conflict, potentially degrading the overall performance of image generation. To solve this issue, this work proposes a \textbf{De}couple-then-\textbf{Me}rge (\textbf{DeMe}) framework, which begins with a pretrained model and finetunes separate models tailored to specific timesteps. We introduce several improved techniques during the finetuning stage to promote effective knowledge sharing while minimizing training interference across timesteps. Finally, after finetuning, these separate models can be merged into a single model in the parameter space, ensuring efficient and practical inference. Experimental results show significant generation quality improvements upon 6 benchmarks including Stable Diffusion on COCO30K, ImageNet1K, PartiPrompts, and DDPM on LSUN Church, LSUN Bedroom, and CIFAR10. Code is available at \href{https://github.com/MqLeet/DeMe}{GitHub}.

==> sec/fig/qualitative_LSUN.tex <==
\begin{figure}[t]
    \centering
    \vspace{-0.1cm}
    \includegraphics[width=1.0\linewidth]{sec/fig/fig-lsun.pdf}
    \vspace{-0.6cm}
    \caption{Qualitative comparison between our method and original DDPM on LSUN. More generated images could be found in supplementary material.
    %\textbf{Upper row} of images are generated by DDPM and \textbf{lower row} of images are generated by our ensemble scheme. %The upper row fail to generate images containing bedroom while the lower row generates bedroom successfully.
    }
    \vspace{-0.5cm}
    \label{fig:qualitive_bedroom}
\end{figure}

==> sec/tabs/rebut-tab1-dit.tex <==
\begin{table}[t]
    \centering
    \vspace{-0.2cm}
    \caption{Results on CIFAR10, CelebA with U-ViT~\textcolor{RoyalBlue}{(a)}, ImageNet with DiT~\textcolor{RoyalBlue}{(c)}. Applications on diffusion pruning~\textcolor{RoyalBlue}{(b)}. Results on LoRA and DeMe on ImageNet~\textcolor{RoyalBlue}{(d)}. Lower FID is better.}
    \vspace{-0.4cm}
    % 第一行（两个子表）
    \begin{subtable}[t]{0.49\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{llll}
        \toprule
        \multirow{1}{*}{\textbf{Method}} & \textbf{CIFAR10} & \textbf{CelebA} & \textbf{\#Iterations} \\
        \midrule
        U-ViT                             & 3.68             & 3.24            & 500K                     \\ 
        \midrule
        P2 Weighting                       & 3.51             & 3.07           & 80K                     \\
        ANT-NashMTL                       & 3.41             & 3.01            & 80K                     \\
        ANT-UW                       & 3.38             & 2.97            & 80K                     \\
        \midrule
        DeMe (Ours) \cellcolor{linecolor1} & \textbf{3.27}$_{~\mathbf{(-0.41)}}$ \cellcolor{linecolor1} & \textbf{2.89}$_{~\mathbf{(-0.35)}}$ \cellcolor{linecolor1} & 20K$\times$4 \cellcolor{linecolor1} \\ 
        \bottomrule
        \end{tabular}
        }
        \caption{}
        \label{tab:rebut_u-vit}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.48\linewidth}
        \centering
        \resizebox{1.1\linewidth}{!}{
        \begin{tabular}{ccccc}
          \toprule
          \multicolumn{5}{c}{\bf DeMe on Diff-Pruning (Fang et al. NeurIPS23)} \\
          \midrule
          \bf \multirow{2}{*}{Pruning Ratios} & \multirow{2}{*}{\bf \#Params} & \multirow{2}{*}{\bf MACs} & \multicolumn{2}{c}{\multirow{1}{*}{\textbf{FID$\downarrow$}}}  \\ \cmidrule{4-5}
          & & & \bf original & \bf DeMe (Ours)
          
          \\ \midrule  
          0\% (Original Model)  & 35.7M & 6.1G &  4.27 & 4.27\cellcolor{linecolor1} \\ % 0.0
          16\% & 27.5M & 5.1G &  4.62 & 4.16$_{~\mathbf{(-0.46)}}$\cellcolor{linecolor1} \\ % 0.2
          44\% & 19.8M & 3.4G &  5.29 & 4.66$_{~\mathbf{(-0.63)}}$\cellcolor{linecolor1} \\ % 0.3
          56\% & 14.3M & 2.7G &  6.36 & 4.84$_{~\mathbf{(-1.52)}}$\cellcolor{linecolor1} \\ % 0.4
          70\% & 8.6M &  1.5G &  9.33 & 6.70$_{~\mathbf{(-2.63)}}$\cellcolor{linecolor1} \\ % 0.6
        \bottomrule
        \end{tabular}
        }
        \caption{}
        \label{tab:rebut_prune}
    \end{subtable}
    
    \vspace{-0.2cm}
    
    % % 第二行（两个子表）
    % \begin{subtable}[t]{0.49\linewidth}
    %     \centering
    %     \resizebox{\linewidth}{!}{
    %     \begin{tabular}{lllll}
    %     \toprule
    %     \textbf{Method} & \textbf{CIFAR10} & \textbf{LSUN-Church} & \textbf{LSUN-Bedroom} & \textbf{\#Iterations} \\
    %     \midrule
    %     DDPM            & 4.42             & 10.69            & 6.46                 & -                     \\
    %     \midrule
    %     SNR+1 w/ LoRA     & 5.11              & 10.47         & 6.49           & 80K  \\
    %     Trun-SNR w/ LoRA     & 4.59              & 10.26       & 6.27             & 80K  \\
    %     Min-SNR-\(\gamma\) w/ LoRA     & 4.11              & 9.90     & 6.03            & 80K     \\
    %     P2 Weighting w/ LoRA     & 4.19              & 9.96           & 6.08        & 80K  \\
    %     \midrule
    %     DeMe (After Merge) \cellcolor{linecolor1} & \textbf{3.51}$_{~\mathbf{(-0.91)}}$ \cellcolor{linecolor1} & \textbf{7.27}$_{~\mathbf{(-3.42)}}$ \cellcolor{linecolor1} & \textbf{5.84}$_{~\mathbf{(-0.62)}}$ \cellcolor{linecolor1} & 20K$\times$4 \cellcolor{linecolor1} \\ 
    %     \bottomrule
    %     \end{tabular}
    %     }
    %     \caption{}
    %     \label{tab:rebut_lora}
    % \end{subtable}


    \begin{subtable}[t]{0.49\linewidth}
        \centering
        \resizebox{\linewidth}{!}{
        \begin{tabular}{lll}
        \toprule
        \textbf{Method}  & \textbf{ImageNet} & \textbf{\#Iterations} \\
        \midrule
        DiT              & 2.88              & 400K                     \\
        \midrule
        P2 Weighting     & 2.84              & 80K                      \\
        ANT-NashMTL      & 2.77              & 80K                      \\
        ANT-UW           & 2.65              & 80K                      \\
        \midrule
        DeMe (Ours) \cellcolor{linecolor1} & \textbf{2.49}$_{~\mathbf{(-0.39)}}$ \cellcolor{linecolor1} & 20K$\times$4 \cellcolor{linecolor1} \\ 
        \bottomrule
        \end{tabular}
        }
        \caption{}
        \label{tab:rebut_dit}
    \end{subtable}
    \hfill
    \begin{subtable}[t]{0.49\linewidth}
        \centering
        \resizebox{1.1\linewidth}{!}{
        \begin{tabular}{lllll}
            \toprule
            \multirow{1}{*}{\textbf{Method}} & \textbf{FID$\downarrow$}  & & \multirow{1}{*}{\textbf{\#Iterations}} \\  \midrule
            Stable Diffusion            & 27.62                    &                       & -                                      \\ \midrule
            P2 Weighting w/ LoRA               &  27.16                                     &  & 80K                                    \\ 
            ANT-NashMTL  w/ LoRA               &  27.49                                      &  & 80K                                    \\ 
            ANT-UW  w/ LoRA               &    26.98                                 &  & 80K                                    \\ \midrule
            DeMe w/ PPL            &  27.55                                     &  & 80K                                    \\ \midrule
            DeMe (Ours) w/ CL \cellcolor{linecolor1}            & 26.36$_{~(-1.26)}$ \cellcolor{linecolor1}              &  \cellcolor{linecolor1}                     & 20K$\times$4 \cellcolor{linecolor1}                                                               \\ \bottomrule
        \end{tabular}
        }
        \caption{}
        \label{tab:rebut_lora}
    \end{subtable}
    \vspace{-1.0cm}
\end{table}
